Neural networks with linear threshold activations: structure and algorithms

In this article we present new results on neural networks with linear threshold activation functions. We precisely characterize the class of functions that are representable by such neural networks and show that 2 hidden layers are necessary and sufficient to represent any function representable in the class. This is a surprising result in the light of recent exact representability investigations for neural networks using other popular activation functions like rectified linear units (ReLU). We also give precise bounds on the sizes of the neural networks required to represent any function in the class. Finally, we design an algorithm to solve the empirical risk minimization (ERM) problem to global optimality for these neural networks with a fixed architecture. The algorithm's running time is polynomial in the size of the data sample, if the input dimension and the size of the network architecture are considered fixed constants. The algorithm is unique in the sense that it works for any architecture with any number of layers, whereas previous polynomial time globally optimal algorithms work only for very restricted classes of architectures. Using these insights, we propose a new class of neural networks that we call shortcut linear threshold networks. To the best of our knowledge, this way of designing neural networks has not been explored before in the literature. We show that these neural networks have several desirable theoretical properties.

==> commands.tex <==
\tikzset{main node/.style={rectangle,fill=blue!20,draw=none,minimum size=0.3cm,inner sep=3pt, rounded corners = 3pt,font=\sffamily},}

\tikzset{transparent node/.style={circle,fill=white!20,draw,minimum size=0cm,inner sep=0pt},}


\tikzset{%
	>={Latex[width=2mm,length=2mm]},
	% Specifications for style of nodes:
	base/.style = {rectangle, rounded corners, draw=black,
		minimum width=4cm, minimum height=1cm,
		text centered, font=\sffamily, text width=4cm },
	ontology/.style={rectangle, rounded corners, draw=black,
		minimum width=1cm, minimum height=.5cm,
		text centered, font=\sffamily, text width=1cm },
	activityStarts/.style = {base, fill=blue!30},
	entity/.style = {base},
	workflow/.style={rectangle, draw=black,
		minimum width=2cm, minimum height=0.4cm,
		text centered, font=\sffamily, text width=4cm},
	data/.style={rectangle, rounded corners, draw=black,
		minimum width=2cm, minimum height=0.4cm,
		text centered, font=\sffamily, text width=5cm},
	startstop/.style = {base, fill=red!30},
	activityRuns/.style = {base, fill=green!30},
	process/.style = {base, minimum width=2.3cm, fill=orange!15,
		font=\ttfamily},
}



\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}


\DeclareMathOperator{\Ima}{Im}
\newcommand{\statement}[1]{%
	#1\enspace\ignorespaces
}

%\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Data %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def \n {8}
\def \radius {3cm}
\def \smallRadius {2cm}
\def \verySmallRadius {0.95cm}
\def \margin {10} % margin in angles, depends on the radius

\newcounter{mylistcounter}

\def\saveitem#1{%
	\stepcounter{mylistcounter}%
	\expandafter\def\csname mylist\themylistcounter\endcsname{#1}}

\forcsvlist{\saveitem}{%
	31,24,23,43,42,41,34,32,C
}%

\def\getnthelement#1{\csname mylist#1\endcsname}
\newcounter{mylistcounterbis}
\def\saveitembis#1{%
	\stepcounter{mylistcounterbis}%
	\expandafter\def\csname mylistbis\themylistcounterbis\endcsname{#1}}

\forcsvlist{\saveitembis}{%
	341, 342, 423, 234, 432, 324, 431, C
}%

\def\getnthelementbis#1{\csname mylistbis#1\endcsname}

\def \nthird {9}
\newcounter{mylistcounterthird}
\def\saveitemthird#1{%
	\stepcounter{mylistcounterthird}%
	\expandafter\def\csname mylistthird\themylistcounterthird\endcsname{#1}}

\forcsvlist{\saveitemthird}{%
	14,24,41,12,23,33,13,21,42, C
}%

\def\getnthelementthird#1{\csname mylistthird#1\endcsname}
\newcounter{mylistcounterfourth}
\def\saveitemfourth#1{%
	\stepcounter{mylistcounterfourth}%
	\expandafter\def\csname mylistfourth\themylistcounterfourth\endcsname{#1}}

\forcsvlist{\saveitemfourth}{%
	213,133,233,123,412,241,124, 214, 421, 142, C
}%

\def\getnthelementfourth#1{\csname mylistfourth#1\endcsname}

\newcommand{\Def}[1]{{\bfseries #1}}

\newcommand{\Draft}[1]{#1}
\newcommand{\YP}[1]{\Draft{\todo[color=blue!10]{\sffamily yann: #1}}}
\newcommand{\YPi}[1]{\Draft{\todo[inline, color=blue!10]{\sffamily yann: #1}}}
\newcommand{\SK}[1]{\Draft{\todo[inline, color=green!80!black!10]{\sffamily sammy: #1}}}
%\renewcommand{\Draft}[1]{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand\equalhat{\mathrel{\stackon[1.5pt]{=}{\stretchto{\scalerel*[\widthof{=}]{\wedge}{\rule{1ex}{3ex}}}{0.5ex}}}}

\newcommand{\specialcell}[2][c]{%
	\begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

%\pgfplotsset{compat=1.16}



==> figure_BraidArrangement.tex <==
\begin{figure}[htbp]
    \centering
	\begin{tikzpicture}
		\draw (-4,0)--(4,0);
		\draw(-2,-3.4641)--(2,3.4641);
		\draw(-2,3.4641)--(2,-3.4641);

		\node[] ()at(2,1.5){$x_1<x_2<x_3$};
        \node[] ()at(2,1){$B_3(x)=1$};
		\node[] ()at(0,2.5){$x_1<x_3<x_2$};
        \node[] ()at(0,2){$B_3(x)=0$};
		\node[] ()at(-2,1.5){$x_3<x_1<x_2$};
        \node[] ()at(-2,1){$B_3(x)=1$};
		\node[] ()at(-2,-1){$x_3<x_2<x_1$};
        \node[] ()at(-2,-1.5){$B_3(x)=0$};
		\node[] ()at(0,-2){$x_2<x_3<x_1$};
        \node[] ()at(0,-2.5){$B_3(x)=1$};
		\node[] ()at(2,-1){$x_2<x_1<x_3$};
        \node[] ()at(2,-1.5){$B_3(x)=0$};

		\node[] ()at(5,0){$x_1=x_2$};
		\node[] ()at(3,4){$x_2=x_3$};
		\node[] ()at(-3,4){$x_1=x_3$};
	\end{tikzpicture}
	\caption{An example of $B_3(x)$ which is projected to the plane $x+y+z=0$.}
	\label{fig:BraidArrangement}
\end{figure}

==> figure_ContinuousParity.tex <==
\begin{figure}[htbp]
    \centering
	\begin{tikzpicture}
		[InputNode/.style={circle,fill=blue!20,thick, minimum size=10pt},
		HiddenNode/.style={circle,fill=red!20,thick, minimum size=10pt},
        OutputNode/.style={circle,fill=green!20,thick, minimum size=10pt}]

		\node[]()at(-1,0){Input layer};
		\node[]()at(-1,-2){Hidden layers};
		\node[]()at(-1,-13){Output layer};

		\foreach \x in {1,...,4}  
		\node[InputNode] (a_\x) at (\x,0){};  
        \node[](cdots) at (5,0) {$\cdots$};
        \node[InputNode] (a_5) at (6,0){};
		\node[InputNode] (a_6) at (7,0){};
		
		\foreach \z in {1,...,4}
		\node[HiddenNode] (b_\z) at (\z, -2){};
		\node[](cdots) at (5,-2) {$\cdots$};
        \node[HiddenNode] (b_5) at (6,-2){};
		\node[HiddenNode] (b_6) at (7,-2){};

        \foreach \i in {1,...,6}
        \draw[-stealth] (a_\i)--(b_\i);
        \node[]()at(1-0.25,-1){$1$};
		\node[]()at(2-0.25,-1){$1$};
		\node[]()at(3-0.25,-1){$1$};
		\node[]()at(4-0.25,-1){$1$};
		\node[]()at(6-0.25,-1){$1$};
        \node[]()at(7-0.25,-1){$1$};
		
		% Second hidden layer
		\foreach \z in {1,...,4}
		\node[HiddenNode] (c_\z) at (\z, -4){};
		\node[](cdots) at (5,-4) {$\cdots$};
        \node[HiddenNode] (c_5) at (6,-4){};
		\node[HiddenNode] (c_6) at (7,-4){};

		% Connections between the second hidden layer and the third hidden layer
		\draw[-stealth,draw=blue] (b_1)--(c_1);
		\draw[-stealth,draw=blue] (b_1)--(c_2);
		\draw[-stealth,draw=red] (b_2)--(c_1);
		\draw[-stealth,draw=red] (b_2)--(c_2);
		
		\draw[-stealth,draw=blue] (b_3)--(c_3);
		\draw[-stealth,draw=blue] (b_3)--(c_4);
		\draw[-stealth,draw=red] (b_4)--(c_3);
		\draw[-stealth,draw=red] (b_4)--(c_4);
		
		\draw[-stealth,draw=blue] (b_5)--(c_5);
		\draw[-stealth,draw=blue] (b_5)--(c_6);
		\draw[-stealth,draw=red] (b_6)--(c_5);
		\draw[-stealth,draw=red] (b_6)--(c_6);
        
		\node[] ()at(1-0.25,-3) {\textcolor{blue}{$-1$}};
		\node[] ()at(1+0.25,-3) {\textcolor{blue}{$1$}};
		\node[] ()at(2-0.25,-3) {\textcolor{red}{$1$}};
		\node[] ()at(2+0.25,-3) {\textcolor{red}{$-1$}};

		\node[] ()at(3-0.25,-3) {\textcolor{blue}{$-1$}};
		\node[] ()at(3+0.25,-3) {\textcolor{blue}{$1$}};
		\node[] ()at(4-0.25,-3) {\textcolor{red}{$1$}};
		\node[] ()at(4+0.25,-3) {\textcolor{red}{$-1$}};

		\node[] ()at(6-0.25,-3) {\textcolor{blue}{$-1$}};
		\node[] ()at(6+0.25,-3) {\textcolor{blue}{$1$}};
		\node[] ()at(7-0.25,-3) {\textcolor{red}{$1$}};
		\node[] ()at(7+0.25,-3) {\textcolor{red}{$-1$}};


		% Third hidden layer
		\node[HiddenNode] (d_2) at (2, -6){};
		\node[HiddenNode] (d_4) at (4, -6){};
		\node[HiddenNode] (d_6) at (7, -6){};
		\node[](cdots) at (5,-6) {$\cdots$};


		% Connections between the third hidden layer and the forth hidden layer
		\draw[-stealth] (c_1)--(d_2);
		\draw[-stealth] (c_2)--(d_2);
		\draw[-stealth] (c_3)--(d_4);
		\draw[-stealth] (c_4)--(d_4);
		\draw[-stealth] (c_5)--(d_6);
		\draw[-stealth] (c_6)--(d_6);
		
		\node[] ()at(1+0.25,-5){$1$};
		\node[] ()at(2+0.25,-5){$1$};
		\node[] ()at(3+0.25,-5){$1$};
		\node[] ()at(4+0.25,-5){$1$};
		\node[] ()at(6+0.25,-5){$1$};
		\node[] ()at(7+0.25,-5){$1$};

		% Forth hidden layer (some dots)
		\node[]()at(2,-7.25){$\vdots$};
		\node[]()at(4,-7.25){$\vdots$};
		\node[]()at(7,-7.25){$\vdots$};

		% The second last hidden layer
		\node[HiddenNode] (e_4)at(4,-9){};
		\node[HiddenNode] (e_6)at(6,-9){};

		% The last hidden layer
		\node[HiddenNode] (f_5)at(5,-11){};
		\draw[-stealth] (e_4)--(f_5);
		\draw[-stealth] (e_6)--(f_5);
		\node[] ()at(4,-10){$-1$};
		\node[] ()at(6,-10){$-1$};

		% The output layer
		\node[OutputNode] (output)at(5,-13){};
		\draw[-stealth] (f_5)--(output);
		\node[] ()at(4.5,-12){$1$};

		%\node[HiddenNode] (g_1)at(4,-12){};
		%\node[HiddenNode] (g_2)at(5,-12){};
		%\draw[-stealth] (f)--(g_1);
		%\draw[-stealth] (f)--(g_2);
		%\node[] ()at(4.25,-11){$1$};
		%\node[] ()at(5.25,-11){$-1$};

		%\node[OutputNode] (output)at(5,-14){};
		%\draw[-stealth] (g_1)--(output);
		%\draw[-stealth] (g_2)--(output);

		% Input x_1,...,x_n
		\foreach \i in {1,2,3,4}
		{\node[] (x_\i)at(\i,1){$x_\i$};
		\draw[-stealth] (x_\i)--(a_\i);}
		\node[] (x_5)at(6,1){$x_{n-1}$};
		\node[] (x_6)at(7,1){$x_{n}$};
		\draw[-stealth] (x_5)--(a_5);
		\draw[-stealth] (x_6)--(a_6);
	\end{tikzpicture}
	\caption{A linear threshold DNN that implements $p_n(x)$ when $n$ is even. Every neuron in hidden layers has $0$ bias except for the last one, which takes $0.5$ as its bias.}
	\label{fig:ContinuousParity}
\end{figure}


==> figure_ShortcutNeuralNets.tex <==
\begin{figure}[htbp] 
    \centering
	\begin{tikzpicture}
		[InputNode/.style={circle,fill=blue!20,thick, minimum size=10pt},
		HiddenNode/.style={circle,fill=red!20,thick, minimum size=10pt},
        OutputNode/.style={circle,fill=green!20,thick, minimum size=10pt}]

		\node[]()at(-1,0){Input: $x \in \mathbb{R}^{w_0}$};
		\node[]()at(-0.5,-4.5){$x^{(k)} \in \mathbb{R}^{w_k}$};
		\node[]()at(-1,-7){Output: $\langle A^\top x + b , x^{(k)} \rangle$};

		\foreach \i in {3,...,4}  
		\node[InputNode] (a_\i) at (\i,0){};  
        \node[](cdots) at (5,0) {$\cdots$};
        \node[InputNode] (a_5) at (6,0){};

		\foreach \i in {2,...,4}
		\node[HiddenNode] (b_\i) at (\i,-2){};
		\node[](cdots) at (5,-2) {$\cdots$};
		\node[HiddenNode] (b_5) at (6,-2){};
		\node[HiddenNode] (b_6) at (7,-2){};

		\foreach \i in {3,...,5}
			{\foreach \j in {2,...,6}
			\draw[-stealth] (a_\i)--(b_\j);}

		\node[](vdots) at (3,-3.25) {$\vdots$};
		\node[](vdots) at (4,-3.25) {$\vdots$};
		\node[](vdots) at (5,-3.25) {$\vdots$};
		\node[](vdots) at (6,-3.25) {$\vdots$};

		\foreach \i in {2,...,4}
			\node[HiddenNode] (c_\i) at (\i,-4.5){};
			\node[](cdots) at (5,-4.5) {$\cdots$};
			\node[HiddenNode] (c_5) at (6,-4.5){};
			\node[HiddenNode] (c_6) at (7,-4.5){};
		
		\node[OutputNode] (output) at (4.5,-7){};

		\foreach \i in {2,...,6}
		\draw[-stealth] (c_\i)--(output);
		
		% Shortcut connection
		\draw[rounded corners, draw=blue!60] (2.5,0.25) rectangle (6.5,-0.25);
		\draw[-stealth,draw=blue!60,rounded corners] (6.5,0)--(8,0)--(8,-6.75)--(4.8,-6.8);
		\node[]() at (8.5,-3.5) {\textcolor{blue!60}{$\qquad A^\top x$}};
	\end{tikzpicture}
	\caption{Illustration of a $\R^{w_0} \rightarrow \R$ shortcut linear threshold neural networks with $k$ hidden layers, where $x{\color{blue} \in \R^{w_0}}$ is the input {\color{blue}to the network}, $x^{(k)} {\color{blue}\in \R^{w_k}}$ is the output of the $k$-th hidden layer. }
	\label{fig:shortcut}
\end{figure}

==> figure_splitting_cubes.tex <==

\newcommand{\Depth}{2}
\newcommand{\Height}{2}
\newcommand{\Width}{2}


\begin{figure}

    \centering
   \scalebox{0.8}{ 
    \subfloat[$\mathcal{A}=\{ \emptyset, \{1\}, \{1,3\}, \{3\}\}$]{
   \begin{tikzpicture}
\coordinate (O) at (0,0,0);

\coordinate (A) at (0,\Width,0);

\coordinate (B) at (0,\Width,\Height);

\coordinate (C) at (0,0,\Height);

\coordinate (D) at (\Depth,0,0);

\coordinate (E) at (\Depth,\Width,0);

\coordinate (F) at (\Depth,\Width,\Height);

\coordinate (G) at (\Depth,0,\Height);

 \draw[->] (0,0,0) -- (3,0,0) node[below]{$x_2$};
 \draw[->] (0,0,0) -- (0,0,3) node[below]{$x_1$};
 \draw[->] (0,0,0) -- (0,3,0) node[left]{$x_3$};


 

\draw[blue,fill=red!10] (O) -- (C) -- (G) -- (D) -- cycle;% Bottom Face
\draw[blue,fill=blue!30] (O) -- (A) -- (E) -- (D) -- cycle;% Back Face
\draw[blue,fill=red!10] (O) -- (A) -- (B) -- (C) -- cycle;% Left Face
\draw[blue,fill=red!20,opacity=0.8] (D) -- (E) -- (F) -- (G) -- cycle;% Right Face
\draw[blue,fill=red!20,opacity=0.6] (C) -- (B) -- (F) -- (G) -- cycle;% Front Face
\draw[blue,fill=red!20,opacity=0.8] (A) -- (B) -- (F) -- (E) -- cycle;% Top Face


 \fill[blue,opacity=0.1] (1,-0.3,0) -- (1,-0.3,2) -- (1,2.3,2) --  (1,2.3,0) -- node[midway,right]{} cycle;
\end{tikzpicture}

    }}
 \scalebox{0.8}{\subfloat[$\mathcal{A}=\{\{1,2\}, \{1,2,3\}\}$]{
   \begin{tikzpicture}
\coordinate (O) at (0,0,0);

\coordinate (A) at (0,\Width,0);

\coordinate (B) at (0,\Width,\Height);

\coordinate (C) at (0,0,\Height);

\coordinate (D) at (\Depth,0,0);

\coordinate (E) at (\Depth,\Width,0);

\coordinate (F) at (\Depth,\Width,\Height);

\coordinate (G) at (\Depth,0,\Height);

 \draw[->] (0,0,0) -- (3,0,0) node[below]{$x_2$};
 \draw[->] (0,0,0) -- (0,0,3) node[below]{$x_1$};
 \draw[->] (0,0,0) -- (0,3,0) node[left]{$x_3$};



\draw[blue,fill=red!10] (O) -- (C) -- (G) -- (D) -- cycle;% Bottom Face
\draw[blue,fill=blue!30] (O) -- (A) -- (E) -- (D) -- cycle;% Back Face
\draw[blue,fill=red!10] (O) -- (A) -- (B) -- (C) -- cycle;% Left Face
\draw[blue,fill=red!20,opacity=0.8] (D) -- (E) -- (F) -- (G) -- cycle;% Right Face
\draw[blue,fill=red!20,opacity=0.6] (C) -- (B) -- (F) -- (G) -- cycle;% Front Face
\draw[blue,fill=red!20,opacity=0.8] (A) -- (B) -- (F) -- (E) -- cycle;% Top Face



 \fill[blue,opacity=0.1] (2,-0.3,0.3) -- (1,-0.3,2) -- (1,2.3,2) --  (2,2.3,0.3) -- node[midway,right]{} cycle;
\end{tikzpicture}

    }}
         \caption{Two linearly separable collections of $2^{\{1, 2, 3\}}$ in $\mathbb{R}^{3}$. The subsets of $\{1, 2, 3\}$ are represented by the vertices of $\{0,1\}^3$. The blue hyperplanes represent a possible separation of the corresponding vertices, giving two different linearly separable collections. }   
    \label{fig:splitting_cubes}


\end{figure}

